The Look-and-Say The Biggest Sequence Eventually Cycles

In this paper we consider a variant of Conway's sequence (OEIS A005150, A006715) defined as follows: the next term in the sequence is obtained by considering contiguous runs of digits, and rewriting them as $ab$ where $b$ is the digit and $a$ is the maximum of $b$ and the run's length. We dub this the "look-and-say the biggest" (LSB) sequence. Conway's sequence is very similar ($b$ is just the run's length). For any starting value except 22, Conway's sequence grows exponentially: the ration of lengths converges to a known constant $\lambda$. We show that LSB does not: for every starting value, LSB eventually reaches a cycle. Furthermore, all cycles have a period of at most 9.

==> img/convergence.tex <==



\begin{tikzpicture}
\begin{semilogxaxis}[legend cell align = left,legend pos = north east,xlabel=$n$,ylabel=$\ell_{n+1}/\ell_n$,width=\textwidth,height=5cm]
\addplot[color=red, mark=+] table[x=i,y=r1] {ratios.dat};
\addlegendentry{$T_0 = 1$};
\addplot[color=blue, mark=x] table[x=i,y=r2] {ratios.dat};
\addlegendentry{$T_0 = 2$};
\addplot[color=green!50!black, mark=x] table[x=i,y=r3] {ratios.dat};
\addlegendentry{$T_0 = d$};
\end{semilogxaxis}

\end{tikzpicture}
